Connecting the Dots: A Knowledgeable Path Generator for Commonsense Question Answering

Commonsense question answering (QA) requires background knowledge which is not explicitly stated in a given context. Prior works use commonsense knowledge graphs (KGs) to obtain this knowledge for reasoning. However, relying entirely on these KGs may not suffice, considering their limited coverage and the contextual dependence of their knowledge. In this paper, we augment a general commonsense QA framework with a knowledgeable path generator. By extrapolating over existing paths in a KG with a state-of-the-art language model, our generator learns to connect a pair of entities in text with a dynamic, and potentially novel, multi-hop relational path. Such paths can provide structured evidence for solving commonsense questions without fine-tuning the path generator. Experiments on two datasets show the superiority of our method over previous works which fully rely on knowledge from KGs (with up to 6% improvement in accuracy), across various amounts of training data. Further evaluation suggests that the generated paths are typically interpretable, novel, and relevant to the task.

==> tables/cases.tex <==
% !TEX root = method.tex
\begin{table*}[t]
\vspace{-0.2cm}
\caption{Generated paths from question entities to gold answer entities.}\label{tab:case}
	\centering
	\scalebox{0.91}{
	\begin{tabular}{l}
		\toprule
		Q1: Where would you find \textbf{magazines} along side many other printed works? \\
		A: doctor. $B^{*}: bookstore$. C: market. D: train station. E: mortuary. \\
		Path from PG-Local: \{magazine, isa, book, atlocation, bookstore\} (2-hop)\\
		Path from PG-Random: \{magazine, \_isa, magazine, atlocation, bookstore\}\\
		\midrule
		%\midrule
		Q2: If you want \textbf{harmony}, what is something you should try to do with the world? \\
		A: take time. B. make noise. C. make war. $D^{*}. make~peace$. E. make haste. \\
		Path from PG-Local: \{harmony, \_hassubevent, make better world, hasprerequisite, make peace\} (2-hop)\\
		Path from PG-Random: \{harmony, \_usedfor, committing perjury, causes, make peace\} \\
		\midrule
		Q3: Janet was watching the \textbf{film} because she liked what? \\
		A: rejection. B: laughter. $C^{*}: being~entertained$. D: fear. E: bordem. \\
		Path from PG-Local: \{film, usedfor, being entertained\} (1-hop)\\
		Path from PG-Random: \{film, \_hascontext, being entertained\} \\	\midrule
		Q4: What do people typically do while playing \textbf{guitar}?\\
		A: cry. B: hear sounds. $C^*: singing$. D:arthritis. E:making music. \\
		Path from PG-Local: \{guitar, usedfor, playing music, \_causes, singing\} (2-hop) \\
		Path from PG-Random: \{guitar, hascontext, music, \_causes, singing\} \\
		\bottomrule
	\end{tabular}
	}
\end{table*}

==> tables/csqa_albert.tex <==
\begin{table}[tb]
\centering
\caption{Classification accuracy on CommonsenseQA  (\citeauthor{lin2019kagnet}'s split) with the reported SoTA system, \textbf{Albert}~\cite{lan2019albert}, as the text encoder.\xiang{update to results on official test.}}
\label{tab:csqa_sota}
\scalebox{0.9}{
\begin{tabular}{lcc}
\toprule
Methods         & Dev           & Test           \\
\midrule
Albert (w/o KG) & 78.26          & 73.98          \\
\midrule
+ RN            & \textbf{79.24} & 73.65          \\
+ RGCN          & 78.46          & {\ul 74.66}    \\
+ GconAttn      & \textbf{79.31} & 73.99          \\
\midrule
+ PG-Local      & 77.56          & 73.33          \\
+ PG-Global     & 78.67          & 74.46          \\
+ PG-Full       & 78.42          & \textbf{76.19} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/csqa_main.tex <==
\begin{table*}[t]
\caption{\small \textbf{Classification accuracy on different proportion of \textit{CommonsenseQA}} (using the data split in \cite{lin2019kagnet}). Results (as mean and standard deviation) are taken from 4 runs of experiments with different random seeds  (top score in boldface, second score underlined).}
\label{tab:csqa_main}
\centering\small
\scalebox{0.9}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Methods}}&
\multicolumn{3}{c}{ \textbf{BERT-large}}&\multicolumn{3}{c}{\textbf{RoBERTa-large}}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& 20\% Train & 60\% Train & 100\% Train & 20\% Train & 60\% Train & 100\% Train\\
\midrule
 Fine-tuned LM (w/o KG) &  $46.25 ~(\pm0.63)$&  $52.30 ~(\pm0.16)$&  $55.39~(\pm0.40)$&$55.28~(\pm0.35)$&$65.56~(\pm0.76)$&$68.69~(\pm0.56)$\\
\midrule
 + RN& $45.12~(\pm0.69)$ &$54.23~(\pm0.28)$  & $\underline{58.92}~(\pm0.14)$ & $61.32~(\pm0.68)$&$66.16~(\pm0.28)$&$69.59~(\pm3.80)$ \\
 + RGCN&  $48.67~(\pm0.28)$& $54.71~(\pm0.37)$ &$57.13~(\pm0.36)$&$58.58~(\pm0.17)$  & $68.33~(\pm0.85)$ &$68.41~(\pm0.66)$\\
 + GconAttn& $47.95~(\pm0.11)$ & $54.96~(\pm0.69)$ &$56.94~(\pm0.77)$  & $57.53~(\pm0.31)$&$68.09~(\pm0.63)$ &$69.88~(\pm0.47)$\\
 %- KVM&  &  &  &  \\
 + Link Prediction& $47.10~(\pm0.79)$ & $53.96~(\pm0.56)$ & $56.02~(\pm0.55)$ & $60.84~(\pm1.36)$&$66.29~(\pm0.29)$&$69.33~(\pm0.98)$ \\
\midrule
 + PathGenerator-Local& $\underline{50.20}~(\pm0.31)$ &$\underline{55.68}~(\pm0.07)$  & $56.81~(\pm0.73)$ & $61.56~(\pm0.72)$&$67.77~(\pm0.83)$&$70.43~(\pm0.65)$ \\
 + PathGenerator-Global& $49.89~(\pm1.03)$ &$55.47~(\pm0.92)$  & $57.21~(\pm0.45)$ & $\underline{62.93}~(\pm0.82)$&$\underline{68.65}~(\pm0.02)$&$\underline{71.55}~(\pm0.99)$\\
 + PathGenerator-Full& $\textbf{51.97}~(\pm0.26)$ &$\textbf{57.53}~(\pm0.19)$  & $\textbf{59.07}~(\pm0.30)$ & $\textbf{63.72}~(\pm0.77)$&$\textbf{69.46}~(\pm0.23)$&$\textbf{72.68}~(\pm0.42)$ \\
\bottomrule
\end{tabular}}
\end{table*}

==> tables/csqa_sota.tex <==
\begin{table}[tb]
\centering
\caption{Classification accuracy on \textit{CommonsenseQA} Official Split (\%). Results for the compared methods are taken from the leaderboard.}
\label{tab:csqa_sota}
\scalebox{0.9}{
\begin{tabular}{lc}
\toprule
Methods         & Test           \\
\midrule
RoBERTa (ensemble) & 72.5 \\
Albert (ensemble) & 76.5          \\
\midrule
UnifiedQA (single) & $\mathbf{79.1}$\\
XLNet + Graph Reasoning (single) & 75.3\\
KEDGN (ensemble) & 74.4\\
RoBERTa + KE (single) & 73.3\\
\midrule
Albert + PG-Full (ensemble)      & $\underline{76.8}$ \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/data_stat.tex <==
% !TEX root = method.tex
\begin{table}[b]
\parbox{.4\linewidth}{
\caption{Statistics of Task Datasets.}\label{tab:data_stat}
	\centering
	\small
	\begin{tabular}{lrrr}
		\toprule
        Dataset & \#Train & \#Dev & \#Test \\
        \midrule
        \textit{CommonsenseQA} &8,767&974&1,221\\
        \textit{OpenBookQA} &4,957 &500 &500 \\
        \bottomrule
	\end{tabular}
}
\quad
\parbox{.7\linewidth}{
\caption{Statistics of Sampled Paths.}\label{tab:path_stat}
    \small
	\centering
	\begin{tabular}{lr}
		\toprule
        Setting & \#Paths \\
        \midrule
        Global &538,766\\
        \textit{CommonsenseQA} &133,612\\
        \textit{OpenBookQA} & 105,155\\
        \bottomrule
	\end{tabular}
}
\end{table}

==> tables/obqa_albert.tex <==
\begin{table}[tb]
\centering
\caption{Classification accuracy on OpenBookQA}
\label{tab:obqa_sota}
\scalebox{0.9}{
\begin{tabular}{lcc}
\toprule
Methods         & Dev           & Test           \\
\midrule
Albert (w/o KG) & 78.26          & 73.98          \\
\midrule
+ RN            & \textbf{79.24} & 73.65          \\
+ RGCN          & 78.46          & {\ul 74.66}    \\
+ GconAttn      & \textbf{79.31} & 73.99          \\
\midrule
+ PG-Local      & 77.56          & 73.33          \\
+ PG-Global     & 78.67          & 74.46          \\
+ PG-Full       & 78.42          & \textbf{76.19} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/obqa_kg_baselines.tex <==

\begin{table}[tb]
\small
\centering
\caption{\textbf{Classification accuracy on \textit{OpenBookQA}}. }
\label{tab:obqa_kg}
\begin{tabular}{lcc}
\toprule
\textbf{Methods}          & \textbf{RoBERTa-large}     & \textbf{AristoRoBERTa}     \\
\midrule
w/o KG          &  64.80   & 78.40       \\
\midrule
+ RN             & $65.20~(\pm1.18)$    &$75.35~(\pm1.39)$
       \\
+ RGCN           & $62.45~(\pm1.57)$   &$74.60~(\pm2.53)$
       \\
+ GconAtten      & $64.75~(\pm1.48)$   &$71.80~(\pm1.21)$
       \\
+ Link Prediction & $66.30~(\pm0.48)$ & $77.25~(\pm1.11)$         \\
\midrule
+ PG-Local       &  $\underline{70.05}~(\pm1.33)$   &$\underline{79.80}~(\pm1.45)$       \\
+ PG-Global      & $68.40~(\pm0.31)$ & $\mathbf{80.05}~(\pm0.68)$         \\
+ PG-Full        & $\textbf{71.20}~(\pm0.96)$ & $79.15~(\pm0.78)$\\
\bottomrule
\end{tabular}
\end{table}

==> tables/obqa_leaderboard.tex <==
\begin{table}[tb]
\centering
\caption{\textbf{Test accuracy on \textit{OpenBookQA}}. Results for the compared methods stem from the leaderboard. Note that the top 2 systems, UnifiedQA (11B parameters) and TTTTT (3B parameters) are too large for an academic setting.}
\label{tab:obqa_sota}
\scalebox{0.9}{
\begin{tabular}{lc}
\toprule
Methods         & Test           \\
\midrule

Careful Selection~\cite{banerjee2019careful} & 72.0\\
AristoRoBERTa & 77.8\\
KF + SIR~\cite{banerjee2020knowledge} & 80.0\\
Albert + KB & 81.0\\
TTTTT\textsuperscript{*}~\cite{raffel2019exploring} & $\underline {83.2}$\\
UnifiedQA\textsuperscript{*}~\cite{khashabi2020unifiedqa} &$\textbf{87.2}$          \\
\midrule
AristoRoBERTa + PG-Full      & $80.2$ \\
Albert + PG-Full & 81.8\\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/obqa_main.tex <==

\begin{table}[tb]
\small
\centering
\caption{\textbf{Classification accuracy on different proportion of training data from \textit{OpenBookQA}}. Standard deviation for 4 runs is omitted due to limited space.\xiang{update to AristoRoberta as encoder; move this one to appendix.}}
\label{tab:obqa_main}
\begin{tabular}{lccc}
\toprule
\textbf{Methods}          & \textbf{20\%}     & \textbf{60\%}    & \textbf{100\%}     \\
\midrule
RoBERTa-large (w/o KG)          & 34.45          & 54.90          & 64.80          \\
\midrule
+ RN             & 44.60          & 62.00          & 65.20          \\
+ RGCN           & 41.35          & 47.20          & 62.45          \\
+ GconAtten      & 41.20          & 55.80          & 64.75          \\
+ Link Prediction & 35.35          & 58.55          & 66.29          \\
\midrule
+ PG-Local       & 48.80          & 60.00          & {\ul 70.47}          \\
+ PG-Global      & {\ul 51.00}    & {\ul 62.95}          & 68.40          \\
+ PG-Full        & \textbf{51.90} & \textbf{63.95} & \textbf{71.20}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/path_stat.tex <==
\begin{table}[tb]
\caption{Statistics of Sampled Paths.}\label{tab:path_stat}
    \small
	\centering
	\begin{tabular}{lr}
		\toprule
        Setting & \#Paths \\
        \midrule
        Global &2,825,692\\
        \textit{CommonsenseQA} &133,612\\
        \textit{OpenBookQA} & 105,155\\
        \bottomrule
	\end{tabular}
\end{table}

==> tables/task_data_stat.tex <==
\begin{table}[t]
\caption{Statistics of Task Datasets.}\label{tab:data_stat}
	\centering
	\small
	\begin{tabular}{lrrr}
		\toprule
        Dataset & \#Train & \#Dev & \#Test \\
        \midrule
        \textit{CommonsenseQA} &8,767&974&1,221\\
        \textit{OpenBookQA} &4,957 &500 &500 \\
        \bottomrule
	\end{tabular}
\end{table}
